PaintSeg: Training-free Segmentation via Painting

The paper introduces PaintSeg, a new unsupervised method for segmenting objects without any training. We propose an adversarial masked contrastive painting (AMCP) process, which creates a contrast between the original image and a painted image in which a masked area is painted using off-the-shelf generative models. During the painting process, inpainting and outpainting are alternated, with the former masking the foreground and filling in the background, and the latter masking the background while recovering the missing part of the foreground object. Inpainting and outpainting, also referred to as I-step and O-step, allow our method to gradually advance the target segmentation mask toward the ground truth without supervision or training. PaintSeg can be configured to work with a variety of prompts, e.g. coarse masks, boxes, scribbles, and points. Our experimental results demonstrate that PaintSeg outperforms existing approaches in coarse mask-prompt, box-prompt, and point-prompt segmentation tasks, providing a training-free solution suitable for unsupervised segmentation.

==> src/archived.tex <==

\begin{table*}[ht]
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
        & &  \multicolumn{3}{c}{DUT-OMRON\cite{yang2013saliency}} & \multicolumn{3}{c}{DUTS-TE \cite{wang2017}} & \multicolumn{3}{c}{ECSSD\cite{shi2016ecssd}} \\
        \cmidrule(rl){3-5}\cmidrule(rl){6-8}\cmidrule(rl){9-11}
         Method & Training & Acc & IoU & max $F_\beta$ & Acc & IoU & max $F_\beta$ & Acc & IoU & max $F_\beta$ \\
        \midrule
        
         \multicolumn{11}{c}{--- \textit{Compared to methods without training} ---} \\
         HS \cite{yan2013hs} &  & .843 & .433 & .561 & .826 & .369 & .504 & .847 & .508 & .673 \\
         wCtr \cite{zhu2014wctr} & & 838 & .416 & .541 & .835 & .392 & .522 & .862 & .517 & .684\\
         WSC \cite{li2015wsc}  & & .865 & .387 & .523 & .862 & .384 & .528 & .852 & .498 & .683\\
         DeepUSPS \cite{nguyen2019deepusps} & & .779 & .305 & .414 & .773 & .305 & .425 & .795 & .440 & .584 \\
         BigBiGAN \cite{voynov2021biggan}  & & .856 & .453 & .549 & .878 & .498 & .608 & .899 & .672 & .782 \\
         E-BigBiGAN \cite{voynov2021biggan}  & & .860 & .464 & .563 & .882 & .511 & .624 & .906 & .684 & .797 \\
         Melas-Kyriazi et al. \cite{melas2021}  & & .883 & .509 & --- & .893 & .528 & - & .915 & .713 & --- \\
         LOST \cite{simeoni2021lost} & & .797 & .410 & .473 & .871 & .518 & .611 & .895 & .654 & .758 \\
         LOST \cite{simeoni2021lost} + BL \cite{barron2016fast} & &.818 &.489 &.578 &.887 &.572 &.697 &.916 &.723 &.837 \\
         DSS \cite{melas2022deepsectralmethod}\cite{wang2022tokencut}& & --- & .567 & --- & --- & .514 & --- & --- & .733 & --- \\
         TokenCut \cite{wang2022tokencut} & & .880 & .533 & {.600} & .903 & .576 & .672 & .918 & .712 & .803 \\
         TokenCut \cite{wang2022tokencut} + BL \cite{barron2016fast}  & & {.897} & \bf{.618} & \bf{.697} & {.914} &.624 & {.755} & {.934} &.772 & {.874} \\
         SelfMask \cite{shin2022selfmask} & & .811 & .403 & - & .845 & .466 & - & .893 & .646 & - \\
         Found \cite{simeoni2022unsupervised} & & - & - & - & - & - & - & .909 & .717 & .792 \\
         TokenCut \cite{wang2022tokencut} + \bf PaintSeg (Ours) & & \bf{.898} & {.610} & {.683} & \bf{.923} & \bf{.670} & \bf{.768} & \bf{.937} & \bf{.806} & \bf{.886} \\
         
         \multicolumn{11}{c}{--- \textit{Compared to methods with training} ---} \\
         SelfMask \cite{shin2022selfmask} & \checkmark & {.901} & .582 & --- & {.923} & {.626} & --- & \bf{.944} & {.781} & --- \\
         FOUND \cite{simeoni2022unsupervised} & \checkmark & \bf{.920} & {.586} & \bf{.683} & \bf{.939} & {.637} & {.733} & .912 & {.793} & \bf{.946} \\ 
         TokenCut \cite{wang2022tokencut} + \bf PaintSeg (Ours) & & {.898} & \bf{.610} & \bf{.683} & {.923} & \bf{.670} & \bf{.768} & {.937} & \bf{.806} & {.886} \\
         \bottomrule
        \end{tabular}}
        \caption{\textbf{Unsupervised saliency detection.} Performances of our method PaintSeg w.r.t. state-of-the-art methods on the unsupervised saliency detection task. BL denotes the application of the post-processing bilateral solver on the generated masks and the column `Learning' specifies which methods have a training step. Best result per section is highlighted in \bf{bold}.
    }
    \vspace{-5pt}
    \label{tab:saliency-detection}
\end{table*}

==> src/main_results.tex <==
\begin{table*}[t]
  \footnotesize
  \centering
  \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{3.63pt}
  \begin{tabular*}{\textwidth}{l l | c c | c c | c c | c c}
    \thickhline

    \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & 
    \multicolumn{2}{c|}{\textbf{GrabCut}} & \multicolumn{2}{c|}{\textbf{Berkeley}} & \multicolumn{2}{c|}{\textbf{SBD}} & \multicolumn{2}{c}{\textbf{DAVIS}} \\
    \cline{3-10}
    & & \textbf{NoC@85 $ \downarrow $} & \textbf{NoC@90 $ \downarrow $} & \textbf{NoC@85 $ \downarrow $} & \textbf{NoC@90 $ \downarrow $} & \textbf{NoC@85 $ \downarrow $} & \textbf{NoC@90 $ \downarrow $} & \textbf{NoC@85 $ \downarrow $} & \textbf{NoC@90 $ \downarrow $} \\

    \hline

    \rowcolor[gray]{0.9}
    \multicolumn{10}{l}{\emph{Deep Supervised Methods}} \\

    DIOS w/o GC~\cite{xu2016deep} \tiny{$_\text{CVPR16}$} & FCN
    & \underline{8.02} & \underline{12.59} & - & - & \underline{14.30} & \underline{16.79} & \underline{12.52} & \underline{17.11} \\
    DIOS w/ GC~\cite{xu2016deep} \tiny{$_\text{CVPR16}$} & FCN
    & \underline{5.08} & \underline{6.08} & - & - & \underline{9.22} & \underline{12.80} & \underline{9.03} & \underline{12.58} \\
    LD~\cite{li2018interactive} \tiny{$_\text{CVPR18}$} & VGG-19
    & \underline{3.20} & \underline{4.79} & - & - & \underline{7.41} & \underline{10.78} & 5.05 & \underline{9.57} \\
    BRS~\cite{jang2019interactive} \tiny{$_\text{CVPR19}$} & DenseNet
    & \underline{2.60} & \underline{3.60} & - & \underline{5.08} & 6.59 & \underline{9.78} & 5.58 & 8.24 \\
    f-BRS~\cite{sofiiuk2020f} \tiny{$_\text{CVPR20}$} & ResNet-101
    & \underline{2.30} & \underline{2.72} & - & 4.57 & 4.81 & 7.73 & 5.04 & 7.41 \\
    FCA-Net~\cite{lin2020interactive} \tiny{$_\text{CVPR20}$} & ResNet-101
    & - & 2.08 & - & 3.92 & - & - & - & 7.57 \\
    IA+SA~\cite{kontogianni2020continuous} \tiny{$_\text{ECCV20}$} & ConvNet
    & - & \underline{3.07} & - & \underline{4.94} & - & - & 5.16 & - \\
    CDNet~\cite{chen2021conditional} \tiny{$_\text{ICCV21}$} & ResNet-34
    & 1.86 & 2.18 & 1.95 & 3.27 & 5.18 & 7.89 & 5.00 & 6.89 \\ 
    RITM~\cite{sofiiuk2022reviving} \tiny{$_\text{ICIP22}$} & HRNet-18
    & 1.76 & 2.04 & 1.87 & 3.22 & 3.39 & 5.43 & 4.94 & 6.71 \\
    FocalClick~\cite{chen2022focalclick} \tiny{$_\text{CVPR22}$} & MiT-B0 
    & 1.66 & 1.90 & - & 3.14 & 4.34 & 6.51 & 5.02 & 7.06 \\
    FocusCut~\cite{lin2022focuscut} \tiny{$_\text{CVPR22}$} & ResNet-101
    & 1.46 & 1.64 & 1.81 & 3.01 & 3.40 & 5.31 & 4.85 & 6.22 \\
    PseudoClick~\cite{liu2022pseudoclick} \tiny{$_\text{ECCV22}$} & HRNet-32
    & - & 1.84 & - & 2.98 & - & 5.61 & 4.74 & 6.16 \\
    SimpleClick~\cite{liu2022simpleclick} \tiny{$_\text{arXiv22}$} & ViT-B 
    & \textbf{1.40} & \textbf{1.54} & \textbf{1.44} & \textbf{2.46} & \textbf{3.28} & \textbf{5.24} & \textbf{4.10} & \textbf{5.48} \\

    \hline

    \hline
    \hline

    \rowcolor[gray]{0.9}
    \multicolumn{10}{l}{\emph{Non-deep Learning Methods}} \\

    GraphCut~\cite{boykov2001interactive} \tiny{$_\text{ICCV01}$} & N/A
    & 7.98 & 10.00 & - & 14.22 & 13.60 & 15.96 & 15.13 & 17.41 \\
    Random Walk~\cite{grady2006random} \tiny{$_\text{TPAMI06}$} & N/A
    & 11.36 & 13.77 & - & 14.02 & 12.22 & 15.04 & 16.71 & 18.31 \\
    Geodesic Matting~\cite{bai2007geodesic} \tiny{$_\text{IJCV09}$} & N/A
    & 13.32 & 14.57 & - & 15.96 & 15.36 & 17.60 & 18.59 & 19.50 \\
    GSC~\cite{gulshan2010geodesic} \tiny{$_\text{CVPR10}$} & N/A
    & 7.10 & 9.12 & - & 12.57 & 12.69 & 15.31 & 15.35 & 17.52 \\
    ESC~\cite{gulshan2010geodesic} \tiny{$_\text{CVPR10}$} & N/A
    & 7.24 & 9.20 & - & 12.11 & 12.21 & 14.86 & 15.41 & 17.70 \\

    \rowcolor[gray]{0.9}
    \multicolumn{10}{l}{\emph{Deep Unsupervised Methods}} \\

    TokenCut$^\star$~\cite{wang2022self} {\tiny{$_\text{CVPR22}$}} & ViT-B
    & 3.04 & 5.74 & 6.30 & 9.97 & 10.82 & 13.16 & 10.56 & 15.01 \\
    FreeMask$^\star$~\cite{wang2022freesolo} {\tiny{$_\text{CVPR22}$}} & ViT-B
    & 4.06 & 6.10 & 5.55 & 9.02 & 8.61 & 12.01 & 8.26 & 13.05 \\
    DSM$^\star$~\cite{melas2022deep} {\tiny{$_\text{CVPR22}$}} & ViT-B
    & 3.64 & 4.64 & 5.49 & 7.75 & 8.59 & 11.57 & 7.08 & 10.11 \\

    \hline

    \rowcolor{aliceblue!80}
    MIS w/o $ \mathcal{L}_{smooth} $ (\emph{Ours}) & ViT-B 
    & 2.08 & 2.56 & 3.40 & 5.51 & 7.38 & 9.92 & 6.78 & 10.08 \\

    \rowcolor{aliceblue!80}
    MIS (\emph{Ours}) & ViT-B 
    & \textbf{1.94} & \textbf{2.32} & \textbf{3.09} & \textbf{4.58} & \textbf{6.91} & \textbf{9.51} & \textbf{6.33} & \textbf{8.44} \\
    
    \thickhline
  \end{tabular*}
  \vspace{1pt}
  \caption{
        \textbf{Comparison with previous methods and baselines on four interactive segmentation benchmarks.}
        $ \star $ denotes baselines that we introduce from other unsupervised tasks.
        From top to bottom we show the previous deep supervised method, unsupervised non-deep learning method, and our newly proposed deep unsupervised method.
        All models listed here are trained on SBD dataset.
        Our MIS achieves superior performance within unsupervised methods and baselines and even exceeds early deep supervised methods (denoted by \underline{underline}).
    }
  \label{tab:main}
\end{table*}

